Intra Order-preserving Functions for Calibration of Multi-Class Neural Networks

Predicting calibrated confidence scores for multi-class deep networks is important for avoiding rare but costly mistakes. A common approach is to learn a post-hoc calibration function that transforms the output of the original network into calibrated confidence scores while maintaining the network's accuracy. However, previous post-hoc calibration techniques work only with simple calibration functions, potentially lacking sufficient representation to calibrate the complex function landscape of deep networks. In this work, we aim to learn general post-hoc calibration functions that can preserve the top-k predictions of any deep network. We call this family of functions intra order-preserving functions. We propose a new neural network architecture that represents a class of intra order-preserving functions by combining common neural network components. Additionally, we introduce order-invariant and diagonal sub-families, which can act as regularization for better generalization when the training data size is small. We show the effectiveness of the proposed method across a wide range of datasets and classifiers. Our method outperforms state-of-the-art post-hoc calibration methods, namely temperature scaling and Dirichlet calibration, in several evaluation metrics for the task.

==> tables/DebiasedECE_MarginalCError_SHORT.tex <==
\begingroup
\setlength{\tabcolsep}{2pt}
\begin{table*}[h]
\begin{center}
\begin{minipage}{.59\linewidth}
\caption{\label{tbl:debiased_ece_paper}\footnotesize{Debiased ECE~\protect\citeRef{kumar2019calibration}}}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c c | c c c c | c c c}
\toprule
Dataset  & Model & Uncal. & TS & \dirodir & \msodir & \dgfn & \oinv & \opre \\
\hline
CIFAR-10     & ResNet 110          & $0.091_7$ & $0.019_4$ & $0.019_5$ & $0.017_3$ & $0.016_2$ & ${\bf 0.000}_1$ & $0.023_6$ \\
CIFAR-10     & Wide ResNet 32      & $0.087_7$ & $0.008_2$ & $0.009_3$ & $0.010_4$ & $0.017_6$ & ${\bf 0.002}_1$ & $0.011_5$ \\
CIFAR-10     & DenseNet 40         & $0.103_7$ & $0.012_2$ & $0.012_3$ & $0.013_4$ & ${\bf 0.011}_1$ & $0.024_6$ & $0.023_5$ \\
\hline 
SVHN         & ResNet 152 (SD)     & $0.019_5$ & $0.009_2$ & $0.010_4$ & $0.009_3$ & ${\bf 0.006}_1$ & $0.023_6$ & $0.034_7$ \\
\hline
CIFAR-100    & ResNet 110          & $0.227_7$ & $0.020_2$ & $0.028_3$ & $0.031_5$ & $0.056_6$ & ${\bf 0.006}_1$ & $0.029_4$ \\
CIFAR-100    & Wide ResNet 32      & $0.248_7$ & $0.010_2$ & $0.019_5$ & $0.030_6$ & $0.015_4$ & ${\bf 0.005}_1$ & $0.014_3$ \\
CIFAR-100    & DenseNet 40         & $0.265_7$ & ${\bf 0.000}_1$ & ${\bf 0.000}_1$ & $0.028_6$ & ${\bf 0.000}_1$ & $0.004_4$ & $0.013_5$ \\
\hline
CARS         & ResNet 50 (pre)     & $0.023_6$ & $0.009_2$ & $0.025_7$ & $0.016_4$ & ${\bf 0.000}_1$ & $0.016_5$ & $0.014_3$ \\
CARS         & ResNet 101 (pre)    & $0.022_6$ & $0.020_3$ & $0.024_7$ & $0.015_2$ & $0.020_4$ & $0.021_5$ & ${\bf 0.013}_1$ \\
CARS         & ResNet 101          & $0.043_5$ & $0.027_3$ & ${\bf 0.015}_1$ & $0.037_4$ & $0.025_2$ & $0.048_6$ & $0.048_7$ \\
\hline
BIRDS        & ResNet 50 (NTS)     & $0.471_7$ & $0.041_4$ & $0.055_5$ & $0.072_6$ & ${\bf 0.015}_1$ & $0.017_2$ & $0.031_3$ \\
\hline
ImageNet     & ResNet 152          & $0.077_7$ & $0.022_4$ & $0.052_5$ & $0.061_6$ & ${\bf 0.001}_1$ & $0.009_2$ & $0.018_3$ \\
ImageNet     & DenseNet 161        & $0.066_7$ & $0.020_4$ & $0.045_5$ & $0.049_6$ & ${\bf 0.010}_1$ & $0.012_2$ & $0.019_3$ \\
ImageNet     & PNASNet5 large      & $0.068_6$ & $0.096_7$ & $0.057_5$ & $0.036_4$ & $0.013_3$ & ${\bf 0.007}_1$ & $0.013_2$ \\
\midrule
\multicolumn{2}{c|}{Avgerage Relative Error} & $1.000_7$    & $0.357_3$    & $0.430_6$    & $0.409_5$    & ${\bf 0.213}_1$    & $0.337_2$    & $0.406_4$   \\
\bottomrule
\end{tabular}}
\end{minipage}~~%
\begin{minipage}{.394\linewidth}
\caption{\label{tbl:marginal_ce_papar}\footnotesize{Marginal Calib. Err. $\times 10^{2}$ ~\protect\citeRef{kumar2019calibration}}}
\resizebox{\linewidth}{!}{%
\begin{tabular}{| c c c c | c c c}
%\hlineB{3}
\toprule
Uncal. & TS & \dirodir & \msodir & \dgfn & \oinv & \opre \\
\hline
$0.859_7$ & $0.305_2$ & $0.371_6$ & $0.363_5$ & $0.346_4$ & ${\bf 0.218}_1$ & $0.336_3$  \\
$1.516_7$ & $1.408_3$ & ${\bf 0.410}_1$ & $0.432_2$ & $1.442_6$ & $1.416_5$ & $1.410_4$ \\
$1.132_7$ & $0.602_4$ & ${\bf 0.417}_1$ & $0.583_2$ & $0.601_3$ & $0.729_6$ & $0.686_5$ \\
\hline
$0.227_2$ & $0.245_3$ & $0.426_5$ & $0.541_6$ & ${\bf 0.178}_1$ & $0.387_4$ & $0.691_7$ \\
\hline
$0.315_7$ & ${\bf 0.129}_1$ & $0.185_5$ & $0.233_6$ & $0.144_3$ & $0.141_2$ & $0.151_4$ \\
$0.356_7$ & $0.266_4$ & $0.222_2$ & ${\bf 0.199}_1$ & $0.270_6$ & $0.268_5$ & $0.257_3$ \\
$0.417_7$ & $0.266_6$ & ${\bf 0.222}_1$ & $0.263_5$ & $0.261_4$ & $0.259_3$ & $0.234_2$ \\
\hline
$0.063_6$ & $0.058_2$ & ${\bf 0.035}_1$ & $0.090_7$ & $0.060_5$ & $0.059_3$ & $0.059_3$ \\
$0.043_3$ & $0.044_4$ & $0.044_4$ & $0.092_7$ & $0.041_2$ & ${\bf 0.034}_1$ & $0.046_6$ \\
${\bf 0.114}_1$ & ${\bf 0.114}_1$ & $0.173_6$ & $0.230_7$ & ${\bf 0.114}_1$ & $0.118_5$ & $0.117_4$ \\
\hline
$0.934_7$ & $0.139_4$& $0.148_6$ & $0.141_5$ & $0.138_3$ & $0.132_2$ & ${\bf 0.130}_1$ \\
\hline
$0.040_6$ & $0.038_2$ & ${\bf 0.034}_1$ & $0.042_7$ & $0.038_2$ & $0.038_2$ & $0.038_2$ \\
$0.041_7$ & $0.039_3$ & ${\bf 0.035}_1$ & $0.038_2$ & $0.039_3$ & $0.039_3$ & $0.039_3$ \\
$0.039_7$ & $0.032_6$ & ${\bf 0.025}_1$ & $0.028_2$ & $0.028_2$ & $0.029_4$ & $0.030_5$ \\
\midrule
$1.000_7$ & $0.750_3$ & $0.735_2$ & $0.996_6$ & ${\bf 0.725}_1$ & $0.778_4$ & $0.898_5$  \\     
\bottomrule
\end{tabular}}
\end{minipage}
\end{center}
\end{table*}
\endgroup

==> tables/ECE_ENS_Best.tex <==
%%%%%%%%%%%%
\begin{table*}[t]
	\begin{center}
	    \caption{\em \label{tbl:ece}\small{ECE (with $M=15$ bins) on various image classification datasets and models with different calibration methods. The subscript numbers represent the rank of the corresponding method on the given model/dataset. The accuracy of the uncalibrated model is shown in parentheses. The number in parentheses in Dir-ODIR and MS methods show the relative change in accuracy for each method.}}
		\resizebox{1.0\linewidth}{!}{%
			\begin{tabular}{c c | c c c c | c c c|c}
				\toprule
				Dataset  & Model & Uncalibrated & Temp. Scaling & \dirodir & \msodir & \dgfn & \oinv & \opre & \uncons \\
				\hline
				CIFAR10 & ResNet~110 & $0.04750_7 (93.56\%)$ & $0.01132_5$ & $0.01086_4 (-0.05\%)$ & $0.01059_3 (-0.05\%)$ & $0.00669_2$ & ${\bf 0.00608}_1$ & $0.01188_6$ & $0.01703 (93.24\%)$ \\
				CIFAR10 & Wide ResNet~32 & $0.04505_7 (93.93\%)$ & $0.00784_4$ & $0.00837_5 (+0.31\%)$ & $0.00727_2 (+0.26\%)$ & $0.01358_6$ & ${\bf 0.00644}_1$ & $0.00772_3$ & $0.00965 (93.81\%)$ \\
				CIFAR10 & DenseNet~40 & $0.05500_7 (92.42\%)$ & $0.00946_2$ & $0.01097_4 (+0.05\%)$ & $0.00988_3 (+0.08\%)$ & ${\bf 0.00691}_1$ & $0.01157_5$ & $0.01283_6$ & $0.01252 (91.88\%)$\\
				\hline
				SVHN & ResNet~152 (SD) & $0.00862_7 (98.15\%)$ & $0.00607_4$ & $0.00582_2 (+0.04\%)$ & $0.00604_3 (-0.00\%)$ & ${\bf 0.00566}_1$ & $00.01161_5$ & $0.01175_6$ & $0.08111 (98.13\%)$\\
				\hline
				CIFAR100 & ResNet~110 & $0.18480_7 (71.48\%)$ & $0.02380_2$ & $0.02822_5 (+0.16\%)$ & $0.02735_4 (+0.07\%)$ & $0.05073_6$ & ${\bf 0.01188}_1$ & $0.02525_3$ & $0.03464 (67.11\%)$\\
				CIFAR100 & Wide ResNet~32 & $0.18784_7 (73.82\%)$ & $0.01472_2$ & $0.01891_5(+0.11\%)$ & $0.02581_6(+0.12\%)$ & $0.01715_3$ & ${\bf 0.01255}_1$ & $0.01733_4$ & $0.04209 (67.71\%)$ \\
				CIFAR100 & DenseNet~40 & $0.21156_7 (70.00\%)$ & $0.00902_2$ & $0.01138_4 (+0.13\%)$ & $0.02197_6(+0.39\%)$ & ${\bf 0.00748}_1$ & $0.00983_3$ & $0.01540_5$ & $0.09901 (57.13\%)$\\
				\hline
				CARS & ResNet~50 (pretrained) & $0.02385_6 (91.25\%)$ & $0.01441_3$ & $0.02433_7 (+0.17\%)$ & $0.01862_5(-0.30\%)$ & $0.01052_2$ & ${\bf 0.01027}_1$ & $0.01854_4$ & $0.01822 (87.79\%)$\\
				CARS & ResNet~101 (pretrained) & $0.02183_6 (92.19\%)$ & $0.01647_4$ & $0.02248_7 (-0.03\%)$ & $0.01911_5(-0.75\%)$ & ${\bf 0.01018}_1$ & $0.01345_3$ & $0.01245_2$ & $0.01547 (88.33\%)$\\
				CARS & ResNet~101 & $0.04206_7 (85.15\%)$ & $0.03007_3$ & $0.02448_2 (-0.30\%)$ & $0.03449_5(-1.09\%)$ & ${\bf 0.02064}_1$ & $0.03229_4$ & $0.03583_6$ & $0.02357 (78.23\%)$ \\
				\hline
				BIRDS & ResNet~50 (NTSNet) & $0.07138_7 (87.43\%)$ & $0.03186_4$ & $0.04860_5 (-0.24\%)$ & $0.05847_6 (-1.10\%)$ & $0.01878_2$ & ${\bf 0.01723}_1$ & $0.02922_3$ & $0.02758 (85.16\%)$\\
				\hline 
				ImageNet & ResNet~152 & $0.06543_7 (76.20\%)$ & $0.02079_4$ & $0.04515_5 (+0.08\%)$ & $0.05667_6 (+0.12\%)$ & ${\bf 0.00873}_1$ & $0.01087_2$ & $0.01670_3$ & $0.12966 (42.83\%)$ \\
				ImageNet & DenseNet~161 & $0.05720_7 (77.05\%)$ & $0.01983_4$ & $0.03736_5 (+0.11\%)$ & $0.04426_6 (+0.40\%)$ & ${\bf 0.01029}_1$ & $0.01233_2$ & $0.01681_3$ & $0.13795 (48.97\%)$\\
				ImageNet & PNASNet5~large & $0.06103_6 (83.09\%)$ & $0.07126_7$ & $0.03979_5 (-0.02\%)$ & $0.02168_4 (+0.27\%)$ & $0.01167_2$ & ${\bf 0.00835}_1$ & $0.01326_3$ & $0.03159 (78.30\%)$\\
				\midrule
%				Avg. Rank &  & 6.79 & 3.57 & 4.64 & 4.57 & \textbf{2.14} & 2.21 & 4.07 \\
				Avg. Rel. Error & & 1.00 & 0.42 & 0.49 & 0.50 & \textbf{0.27} & 0.33 & 0.41 & ? \\
				\bottomrule
			\end{tabular}
		}
	\end{center}
	%\vspace{-.9cm}
\end{table*}

==> tables/NLLCwECE_ENS_BEST_SHORT.tex <==
\begingroup
\setlength{\tabcolsep}{2pt}
\begin{table*}[h]
\begin{center}
\begin{minipage}{.59\linewidth}
\caption{\label{tbl:nll_paper}\footnotesize{NLL}}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c c | c c c c | c c c}
\toprule
Dataset  & Model & Uncal. & TS & \dirodir & \msodir & \dgfn & \oinv & \opre \\
\hline
CIFAR10 & ResNet 110 & $0.358_7$ & $0.209_5$ & $0.205_3$ & ${\bf 0.204}_1$ & $0.207_4$ & $0.205_2$ & $0.210_6$ \\
CIFAR10 & Wide ResNet 32 & $0.382_7$ & $0.192_3$ & $0.182_2$ & ${\bf 0.182}_1$ & $0.192_5$ & $0.192_4$ & $0.193_6$ \\
CIFAR10 & DenseNet 40 & $0.428_7$ & $0.225_3$ & $0.224_2$ & ${\bf 0.222}_1$ & $0.226_4$ & $0.231_6$ & $0.228_5$ \\
\hline
SVHN & ResNet 152 (SD) & $0.085_7$ & ${\bf 0.079}_1$ & ${0.080}_5$ & $0.081_6$ & $0.079_2$ & $0.080_3$ & $0.080_4$ \\
\hline
CIFAR100 & ResNet 110 & $1.693_7$ & $1.092_4$ & $1.096_5$ & ${\bf 1.074}_1$ & $1.101_6$ & $1.080_2$ & $1.084_3$ \\
CIFAR100 & Wide ResNet 32 & $1.802_7$ & $0.945_3$ & $0.953_6$ & ${\bf 0.933}_1$ & $0.949_4$ & $0.943_2$ & $0.950_5$ \\
CIFAR100 & DenseNet 40 & $2.017_7$ & $1.057_2$ & $1.059_3$ & ${\bf 1.050}_1$ & $1.060_4$ & $1.061_5$ & $1.076_6$ \\
\hline
CARS & ResNet~50 (pre) & $0.330_7$ & $0.318_4$ & $0.324_6$ & $0.319_5$ & ${\bf 0.312}_1$ & $0.316_2$ & $0.318_3$ \\
CARS & ResNet~101 (pre) & $0.305_7$ & $0.293_3$ & $0.297_4$ & $0.298_5$ & ${\bf 0.286}_1$ & $0.289_2$ & $0.304_6$ \\
CARS & ResNet~101 & $0.612_7$ & $0.586_4$ & $0.595_6$ & $0.587_5$ & ${\bf 0.574}_1$ & $0.578_2$ & $0.583_3$ \\
\hline
BIRDS & ResNet~50 (NTS) & $0.747_7$ & $0.566_4$ & $0.612_5$ & $0.631_6$ & $0.549_2$ & ${\bf 0.545}_1$ & $0.563_3$ \\
\hline 
ImageNet & ResNet~152 & $0.989_7$ & $0.942_4$ & $0.951_5$ & $0.958_6$ & ${\bf 0.926}_1$ & $0.929_2$ & $0.939_3$ \\
ImageNet & DenseNet~161 & $0.944_7$ & $0.909_5$ & $0.912_6$ & $0.906_3$ & ${\bf 0.889}_1$ & $0.896_2$ & $0.906_4$ \\    
ImageNet & PNASNet5~large & $0.802_7$ & $0.758_6$ & $0.740_5$ & $0.715_4$ & ${\bf 0.656}_1$ & $0.657_2$ & $0.696_3$  \\
\midrule
%Avg. Rank & & $7.00$ & $3.64$ & $4.50$ & $3.29$ & ${\bf 2.64}$ & ${\bf 2.64}$ & $4.29$\\
\multicolumn{2}{c|}{Average Relative Error} & $1.000_7$ & $0.766_4$ & $0.772_6$ & $0.768_5$ & $\mathbf{0.749}_1$ & $0.751_2$ & $0.765_3$ \\
\bottomrule
\end{tabular}}
\end{minipage}~~%
\begin{minipage}{.394\linewidth}
\caption{\label{tbl:cwece_paper}\footnotesize{Classwise-ECE}}
\resizebox{\linewidth}{!}{%
\begin{tabular}{| c c c c | c c c}
%\hlineB{3}
\toprule
Uncal. & TS & \dirodir & \msodir & \dgfn & \oinv & \opre \\
\hline
$0.099_7$ & $0.043_5$ & $0.040_4$ & ${0.036}_2$ & $0.038_3$ & ${\bf 0.035}_1$ & $0.044_6$ \\
$0.095_7$ & $0.048_4$ & $0.030_2$ & ${\bf 0.029}_1$ & $0.055_6$ & $0.048_3$ & $0.049_5$ \\
$0.114_7$ & $0.040_4$ & $0.037_2$ & ${\bf 0.037}_1$ & $0.039_3$ & $0.046_5$ & $0.052_6$ \\
\hline
$0.019_4$ & $0.019_2$ & $0.020_5$ & $0.021_6$ & ${\bf 0.015}_1$ & ${0.019}_3$ & $0.021_7$ \\
\hline
$0.416_7$ & $0.201_3$ & ${\bf 0.186}_1$ & $0.203_5$ & $0.220_6$ & $0.200_2$ & $0.202_4$ \\ 
$0.420_7$ & $0.186_4$ & ${\bf 0.180}_1$ & $0.180_2$ & $0.186_5$ & $0.194_6$ & $0.185_3$ \\
$0.470_7$ & $0.187_3$ & ${0.186}_2$ & $0.191_5$ & ${\bf 0.186}_1$ & $0.199_6$ & $0.188_4$\\
\hline
$0.174_3$ &  $0.185_7$ & $0.171_2$  & $0.183_6$ & ${\bf 0.169}_1$ & $0.182_5$ & $0.176_4$ \\
%$0.169_2$ &  $0.184_7$ & ${\bf 0.166}_1$ & $0.174_4$ & $0.175_6$ & $0.170_3$ & $0.174_5$ \\
$0.165_4$ & $0.172_6$ & $0.159_2$ & $0.174_7$ & $0.167_5$ & $0.164_3$ & ${\bf 0.155}_1$ \\
$0.263_2$ & $0.272_6$ & $0.263_3$ & $0.275_7$ & $0.266_5$ & $0.265_4$ & ${\bf 0.251}_1$ \\
\hline
$0.249_3$ &  $0.264_7$ & ${\bf 0.229}_1$ & $0.256_6$ & $0.251_5$ & $0.251_4$ & $0.240_2$ \\
\hline 
$0.319_7$ & $0.309_4$ & ${\bf 0.301}_1$ & $0.309_5$ & $0.314_6$ & $0.306_3$ & $0.301_2$ \\
$0.310_7$ & $0.303_5$ & ${\bf 0.294}_1$ & $0.298_2$ & $0.307_6$ & $0.303_4$ & $0.300_3$ \\
$0.314_7$ & $0.256_6$ & ${\bf 0.238}_1$ & $0.243_2$ & $0.250_5$ & $0.246_4$ & $0.245_3$  \\
\midrule
%$5.64$ & $4.71$ & ${\bf 2.00}$ & $4.07$ & $4.14$ & $3.79$ & $3.57$ \\
%$5.40$ & $4.87$ & ${\bf 1.93}$ & $4.07$ & $4.27$ & $3.73$ & $3.67$ \\
$1.000_7$ & $0.752_6$ & $\mathbf{0.704}_1$ & $0.734_3$ & $0.729_2$ & $0.740_4$ & $0.743_5$ \\
\bottomrule
\end{tabular}}
\end{minipage}
\end{center}
\end{table*}
\endgroup

==> tables/NLL_ENS_BEST_SHORT.tex <==
\begin{table*}[h]
\begin{center}
\caption{\em \label{tbl:nll}\small{NLL.}}
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{c c | c c c c | c c c}
\toprule
Dataset  & Model & Uncalibrated & Temp. Scaling & \dirodir & \msodir & \dgfn & \oinv & \opre \\
\hline
CIFAR10 & ResNet 110 & $0.358_7$ & $0.209_5$ & $0.205_3$ & ${\bf 0.204}_1$ & $0.207_4$ & $0.205_2$ & $0.210_6$ \\
CIFAR10 & Wide ResNet 32 & $0.382_7$ & $0.192_3$ & $0.182_2$ & ${\bf 0.182}_1$ & $0.192_5$ & $0.192_4$ & $0.193_6$ \\
CIFAR10 & DenseNet 40 & $0.428_7$ & $0.225_3$ & $0.224_2$ & ${\bf 0.222}_1$ & $0.226_4$ & $0.231_6$ & $0.228_5$ \\
\hline
SVHN & ResNet 152 (SD) & $0.085_7$ & ${\bf 0.079}_1$ & ${0.080}_5$ & $0.081_6$ & $0.079_2$ & $0.080_3$ & $0.080_4$ \\
\hline
CIFAR100 & ResNet 110 & $1.693_7$ & $1.092_4$ & $1.096_5$ & ${\bf 1.074}_1$ & $1.101_6$ & $1.080_2$ & $1.084_3$ \\
CIFAR100 & Wide ResNet 32 & $1.802_7$ & $0.945_3$ & $0.953_6$ & ${\bf 0.933}_1$ & $0.949_4$ & $0.943_2$ & $0.950_5$ \\
CIFAR100 & DenseNet 40 & $2.017_7$ & $1.057_2$ & $1.059_3$ & ${\bf 1.050}_1$ & $1.060_4$ & $1.061_5$ & $1.076_6$ \\
\hline
CARS & ResNet~50 (pretrained) & $0.330_7$ & $0.318_4$ & $0.324_6$ & $0.319_5$ & ${\bf 0.312}_1$ & $0.316_2$ & $0.318_3$ \\
CARS & ResNet~101 (pretrained) & $0.305_7$ & $0.293_3$ & $0.297_4$ & $0.298_5$ & ${\bf 0.286}_1$ & $0.289_2$ & $0.304_6$ \\
CARS & ResNet~101 & $0.612_7$ & $0.586_4$ & $0.595_6$ & $0.587_5$ & ${\bf 0.574}_1$ & $0.578_2$ & $0.583_3$ \\
\hline
BIRDS & ResNet~50 (NTSNet) & $0.747_7$ & $0.566_4$ & $0.612_5$ & $0.631_6$ & $0.549_2$ & ${\bf 0.545}_1$ & $0.563_3$ \\
\hline 
ImageNet & ResNet~152 & $0.989_7$ & $0.942_4$ & $0.951_5$ & $0.958_6$ & ${\bf 0.926}_1$ & $0.929_2$ & $0.939_3$ \\
ImageNet & DenseNet~161 & $0.944_7$ & $0.909_5$ & $0.912_6$ & $0.906_3$ & ${\bf 0.889}_1$ & $0.896_2$ & $0.906_4$ \\
ImageNet & PNASNet5~large & $0.802_7$ & $0.758_6$ & $0.740_5$ & $0.715_4$ & ${\bf 0.656}_1$ & $0.657_2$ & $0.696_3$  \\
\midrule
Avg. Rank & & $7.00$ & $3.64$ & $4.50$ & $3.29$ & ${\bf 2.64}$ & ${\bf 2.64}$ & $4.29$\\
Avg. Rel. Error & & 1.000 & 0.766 & 0.772 & 0.768 & \textbf{0.749} & 0.751 & 0.765 \\
\bottomrule
\end{tabular}
}
\end{center}
%\vspace{-.9cm}
\end{table*}

==> tables/NLL_MarginalCE_BEST_SHORT.tex <==
\begingroup
\setlength{\tabcolsep}{2pt}
\begin{table*}[h]
\begin{center}
\begin{minipage}{.59\linewidth}
\caption{\label{tbl:nll_paper}\footnotesize{NLL}}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c c | c c c c | c c c}
\toprule
Dataset  & Model & Uncal. & TS & \dirodir & \msodir & \dgfn & \oinv & \opre \\
\hline
CIFAR10 & ResNet 110 & $0.358_7$ & $0.209_5$ & $0.205_3$ & ${\bf 0.204}_1$ & $0.207_4$ & $0.205_2$ & $0.210_6$ \\
CIFAR10 & Wide ResNet 32 & $0.382_7$ & $0.192_3$ & $0.182_2$ & ${\bf 0.182}_1$ & $0.192_5$ & $0.192_4$ & $0.193_6$ \\
CIFAR10 & DenseNet 40 & $0.428_7$ & $0.225_3$ & $0.224_2$ & ${\bf 0.222}_1$ & $0.226_4$ & $0.231_6$ & $0.228_5$ \\
\hline
SVHN & ResNet 152 (SD) & $0.085_7$ & ${\bf 0.079}_1$ & ${0.080}_5$ & $0.081_6$ & $0.079_2$ & $0.080_3$ & $0.080_4$ \\
\hline
CIFAR100 & ResNet 110 & $1.693_7$ & $1.092_4$ & $1.096_5$ & ${\bf 1.074}_1$ & $1.101_6$ & $1.080_2$ & $1.084_3$ \\
CIFAR100 & Wide ResNet 32 & $1.802_7$ & $0.945_3$ & $0.953_6$ & ${\bf 0.933}_1$ & $0.949_4$ & $0.943_2$ & $0.950_5$ \\
CIFAR100 & DenseNet 40 & $2.017_7$ & $1.057_2$ & $1.059_3$ & ${\bf 1.050}_1$ & $1.060_4$ & $1.061_5$ & $1.076_6$ \\
\hline
CARS & ResNet~50 (pre) & $0.330_7$ & $0.318_4$ & $0.324_6$ & $0.319_5$ & ${\bf 0.312}_1$ & $0.316_2$ & $0.318_3$ \\
CARS & ResNet~101 (pre) & $0.305_7$ & $0.293_3$ & $0.297_4$ & $0.298_5$ & ${\bf 0.286}_1$ & $0.289_2$ & $0.304_6$ \\
CARS & ResNet~101 & $0.612_7$ & $0.586_4$ & $0.595_6$ & $0.587_5$ & ${\bf 0.574}_1$ & $0.578_2$ & $0.583_3$ \\
\hline
BIRDS & ResNet~50 (NTS) & $0.747_7$ & $0.566_4$ & $0.612_5$ & $0.631_6$ & $0.549_2$ & ${\bf 0.545}_1$ & $0.563_3$ \\
\hline 
ImageNet & ResNet~152 & $0.989_7$ & $0.942_4$ & $0.951_5$ & $0.958_6$ & ${\bf 0.926}_1$ & $0.929_2$ & $0.939_3$ \\
ImageNet & DenseNet~161 & $0.944_7$ & $0.909_5$ & $0.912_6$ & $0.906_3$ & ${\bf 0.889}_1$ & $0.896_2$ & $0.906_4$ \\    
ImageNet & PNASNet5~large & $0.802_7$ & $0.758_6$ & $0.740_5$ & $0.715_4$ & ${\bf 0.656}_1$ & $0.657_2$ & $0.696_3$  \\
\midrule
%Avg. Rank & & $7.00$ & $3.64$ & $4.50$ & $3.29$ & ${\bf 2.64}$ & ${\bf 2.64}$ & $4.29$\\
\multicolumn{2}{c|}{Average Relative Error} & $1.000_7$ & $0.766_4$ & $0.772_6$ & $0.768_5$ & $\mathbf{0.749}_1$ & $0.751_2$ & $0.765_3$ \\
\bottomrule
\end{tabular}}
\end{minipage}~~%
\begin{minipage}{.403\linewidth}
\caption{\label{tbl:marginal_ce_papar}\footnotesize{Marginal Calib. Err. $\times 10^{2}$ ~\protect\cite{kumar2019calibration}}}
\resizebox{\linewidth}{!}{%
\begin{tabular}{| c c c c | c c c}
%\hlineB{3}
\toprule
Uncal. & TS & \dirodir & \msodir & \dgfn & \oinv & \opre \\
\hline
$0.859_7$ & $0.305_2$ & $0.371_6$ & $0.363_5$ & $0.346_4$ & ${\bf 0.218}_1$ & $0.336_3$  \\
$1.516_7$ & $1.408_3$ & ${\bf 0.410}_1$ & $0.432_2$ & $1.442_6$ & $1.416_5$ & $1.410_4$ \\
$1.132_7$ & $0.602_4$ & ${\bf 0.417}_1$ & $0.583_2$ & $0.601_3$ & $0.729_6$ & $0.686_5$ \\
\hline
$0.227_2$ & $0.245_3$ & $0.426_5$ & $0.541_6$ & ${\bf 0.178}_1$ & $0.387_4$ & $0.691_7$ \\
\hline
$0.315_7$ & ${\bf 0.129}_1$ & $0.185_5$ & $0.233_6$ & $0.144_3$ & $0.141_2$ & $0.151_4$ \\
$0.356_7$ & $0.266_4$ & $0.222_2$ & ${\bf 0.199}_1$ & $0.270_6$ & $0.268_5$ & $0.257_3$ \\
$0.417_7$ & $0.266_6$ & ${\bf 0.222}_1$ & $0.263_5$ & $0.261_4$ & $0.259_3$ & $0.234_2$ \\
\hline
$0.063_6$ & $0.058_2$ & ${\bf 0.035}_1$ & $0.090_7$ & $0.060_5$ & $0.059_3$ & $0.059_3$ \\
$0.043_3$ & $0.044_4$ & $0.044_4$ & $0.092_7$ & $0.041_2$ & ${\bf 0.034}_1$ & $0.046_6$ \\
${\bf 0.114}_1$ & ${\bf 0.114}_1$ & $0.173_6$ & $0.230_7$ & ${\bf 0.114}_1$ & $0.118_5$ & $0.117_4$ \\
\hline
$0.934_7$ & $0.139_4$& $0.148_6$ & $0.141_5$ & $0.138_3$ & $0.132_2$ & ${\bf 0.130}_1$ \\
\hline
$0.040_6$ & $0.038_2$ & ${\bf 0.034}_1$ & $0.042_7$ & $0.038_2$ & $0.038_2$ & $0.038_2$ \\
$0.041_7$ & $0.039_3$ & ${\bf 0.035}_1$ & $0.038_2$ & $0.039_3$ & $0.039_3$ & $0.039_3$ \\
$0.039_7$ & $0.032_6$ & ${\bf 0.025}_1$ & $0.028_2$ & $0.028_2$ & $0.029_4$ & $0.030_5$ \\
\midrule
$1.000_7$ & $0.750_3$ & $0.735_2$ & $0.996_6$ & ${\bf 0.725}_1$ & $0.778_4$ & $0.898_5$  \\     
\bottomrule
\end{tabular}}
\end{minipage}
\end{center}
\end{table*}
\endgroup
